Atomicity Checking in Linear Time using Vector Clocks

Multi-threaded programs are challenging to write. Developers often need to reason about a prohibitively large number of thread interleavings to reason about the behavior of software. A non-interference property like atomicity can reduce this interleaving space by ensuring that any execution is equivalent to an execution where all atomic blocks are executed serially. We consider the well studied notion of conflict serializability for dynamically checking atomicity. Existing algorithms detect violations of conflict serializability by detecting cycles in a graph of transactions observed in a given execution. The number of edges in such a graph can grow quadratically with the length of the trace making the analysis not scalable. In this paper, we present AeroDrome, a novel single pass linear time algorithm that uses vector clocks to detect violations of conflict serializability in an online setting. Experiments show that AeroDrome scales to traces with a large number of events with significant speedup.

==> exec_macros.tex <==
%!TEX root = main.tex


% Drawing executions. Arguments: # of threads, and execution. 
\newcommand{\execution}[2]{
\scalebox{0.85}{
  \begin{tikzpicture}%
    \foreach \x in {1,...,#1}
    \node[right] at (1.5*\x+0.2,0.25) {$t_{\x}$};
    \draw (1.2,0) -- (#1*1.5+1.3,0);%
    \pgfmathsetmacro{\y}{1};%
    #2%
    \draw (1.2,0) -- (1.2,-0.4*\y);%
    \draw (#1*1.5+1.3,0) -- (#1*1.5+1.3,-0.4*\y);%
    \foreach \x in {2,...,#1}
    \draw[dashed] (1.5*\x-0.3,0) -- (1.5*\x-0.3,-0.4*\y);%
    \draw (1.2,-0.4*\y) -- (#1*1.5+1.3,-0.4*\y);%
  \end{tikzpicture}
}
}

% \figev arguments: thread id, event, variable/lock
\newcommand{\figev}[2]{\node [left] at (1.25,-0.4*\y)  {\pgfmathprintnumber{\y}};%
                    \node at (#1*1.5 + 0.45,-0.4*\y) {$ #2 $};%
                    \pgfmathsetmacro{\y}{\y+1};}
%\orderedeg{t1}{ind1}{off1}{t2}{ind2}{off2} denotes an edge from an event e1
% to an event e2 such that ei appears at indi in the trace and belongs to thread ti.
% off1 and off2 are offsets from the center.
\newcommand{\orderedge}[6]{
  \draw (#1*1.5 + 0.45 + #3, -0.4*#2) edge[-{Latex[length=2mm, width=2mm]},  ->,>=stealth] (#4*1.5 + 0.45 + #6, -0.4*#5);
}

\newcommand{\executionnonumber}[2]{\begin{tikzpicture}%
                             \foreach \x in {1,...,#1}
                               \node[right] at (2*\x+0.5,0.25) {$t_{\x}$};
                             \draw (1.9,0) -- (#1*2+1.6,0);%
                             \pgfmathsetmacro{\z}{1};%
                             #2%
                             \draw (1.9,0) -- (1.9,-0.5*\z);%
                             \draw (#1*2+1.6,0) -- (#1*2+1.6,-0.5*\z);%
                             \foreach \x in {2,...,#1}
                               \draw (2*\x-0.3,0) -- (2*\x-0.3,-0.5*\z);%
                             \draw (1.9,-0.5*\z) -- (#1*2+1.6,-0.5*\z);%
                           \end{tikzpicture}}                    

\newcommand{\figevnonumber}[2]{\node [left] at (1.75,-0.4*\z) {};%
\node [right] at (#1*2 + 0.3,-0.5*\z) {$ #2 $};%
\pgfmathsetmacro{\z}{\z+1};}

% Drawing programs. Arguments: # of threads, and program
\newcommand{\figprogram}[2]{\begin{tikzpicture}%
                              \foreach \x in {1,...,#1}
                                \node at (2.3*\x-1.15,0.25) {$t_{\x}$};
                              \draw (0,0) -- (#1*2.3+0.6,0);% 
                              \pgfmathsetmacro{\y}{1};%
                              #2%
                              \draw (0,0) -- (0,-0.4*\y);% 
                              \draw (#1*2.3+0.6,0) -- (#1*2.3+0.6,-0.4*\y);% 
                              \draw (0,-0.4*\y) -- (#1*2.3+0.6,-0.4*\y);% 
                            \end{tikzpicture}}
% figstmt arguments: thread id, offset, statement
\newcommand{\figstmt}[3]{\node [left] at (-0.15,-0.4*\y) {\pgfmathprintnumber{\y}};%
                      \node[right] at (#1*2.3 + #2*0.3 - 2.15,-0.4*\y) {\texttt{#3}};
                      \pgfmathsetmacro{\y}{\y+1};}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newtheorem{observation}{Observation}

\newcommand{\nil}{\texttt{nil}}

\newcommand{\drawarrow}{\raisebox{2pt}{\scalebox{0.7}{\tikz{ \draw[-{Latex[length=2mm, width=2mm]},  ->,>=stealth](0,0) -- (7mm,0);} }}}

==> macros.tex <==
%!TEX root = main.tex

\makeatletter
\newcommand{\pnrelbar}{%
  \linethickness{\dimen2}%
  \sbox\z@{$\m@th\prec$}%
  \dimen@=1.1\ht\z@
  \begin{picture}(\dimen@,.4ex)
  \roundcap
  \put(0,.2ex){\line(1,0){\dimen@}}
  \put(\dimexpr 0.5\dimen@-.2ex\relax,0){\line(1,1){.4ex}}
  \end{picture}%
}

\newcommand{\precneq}{\mathrel{\vcenter{\hbox{\text{\prec@neq}}}}}
\newcommand{\prec@neq}{%
  \dimen2=\f@size\dimexpr.04pt\relax
  \oalign{%
    \noalign{\kern\dimexpr.2ex-.5\dimen2\relax}
    $\m@th\prec$\cr
    \noalign{\kern-.5\dimen2}
    \hidewidth\pnrelbar\hidewidth\cr
  }%
}
\makeatother

\newenvironment{myparagraph}[1]{\vspace*{0.1in}\noindent{\bf #1.}}{}

% Labels and references
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\itemlabel}[1]{\label{itm:#1}}
\newcommand{\itemref}[1]{\ref{itm:#1}}
\newcommand{\equlabel}[1]{\label{eq:#1}}
\newcommand{\equref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
% \newcommand{\appref}[1]{ the Appendix}

\newcommand{\setofthreads}{\mathsf{Thr}}
\newcommand{\threads}[1]{\setofthreads_{#1}}
\newcommand{\locks}[1]{\mathsf{Locks}_{#1}}
\newcommand{\vars}[1]{\mathsf{Vars}_{#1}}
\newcommand{\events}[1]{\mathsf{Events}_{#1}}
\newcommand{\wevents}[1]{\mathsf{WEvents}_{#1}}
\newcommand{\reads}[1]{\mathsf{Reads}_{#1}}
\newcommand{\writes}[1]{\mathsf{Writes}_{#1}}
\newcommand{\accesses}[1]{\mathsf{Accesses}_{#1}}
\newcommand{\acquires}[1]{\mathsf{Acquires}_{#1}}
\newcommand{\releases}[1]{\mathsf{Releases}_{#1}}
\newcommand{\forks}[1]{\mathsf{Forks}_{#1}}
\newcommand{\joins}[1]{\mathsf{Joins}_{#1}}
% \renewcommand{\next}[1]{\mathsf{next}_{#1}}
\newcommand{\match}[1]{\mathsf{match}_{#1}}
\newcommand{\lheld}[1]{\mathsf{locksHeld}_{#1}}
\newcommand{\last}[1]{\mathsf{last}_{#1}}


\newcommand{\acq}{\mathtt{acq}}
\newcommand{\rel}{\mathtt{rel}}
\newcommand{\rd}{\mathtt{r}}
\newcommand{\wt}{\mathtt{w}}
\newcommand{\fork}{\mathtt{fork}}
\newcommand{\join}{\mathtt{join}}
% \newcommand{\trbegin}{\rhd}
% \newcommand{\trend}{\lhd}
% \newcommand{\trbeginfig}{\texttopcorner\textcorner}
% \newcommand{\trbeginfig}{\;\raisebox{1.3mm}{\rule{0.4pt}{1.14mm}\raisebox{1mm}{\rule{4mm}{0.4pt}}\rule{0.4pt}{1.14mm} } }
% \newcommand{\trendfig}{\;\raisebox{-0.075mm}{\rule{0.4pt}{1.14mm}\rule{4mm}{0.4pt}\rule{0.4pt}{1.14mm} } }
% \newcommand{\trbegintext}{\;\raisebox{0mm}{\rule{1pt}{1.35mm}\raisebox{1mm}{\rule{3mm}{1pt}}\rule{1pt}{1.35mm} } }
% \newcommand{\trendtext}{\;\raisebox{-0.075mm}{\rule{1pt}{1.35mm}\rule{3mm}{1pt}\rule{1pt}{1.35mm} } }
% \newcommand{\trbegin}{{\protect\trbegintext}\!}
% \newcommand{\trend}{{\protect\trendtext}\!}
\newcommand{\trbegin}{\rhd}
\newcommand{\trend}{\lhd}
\newcommand{\trbeginfig}{\rhd}
\newcommand{\trendfig}{\lhd}
\newcommand{\sync}{\mathtt{sync}}
\newcommand{\lk}{\ell}
\newcommand{\ev}[1]{\langle #1\rangle}
\newcommand{\tr}{\sigma}
\newcommand{\conf}{\asymp}
\newcommand{\comp}{\circ}
\newcommand{\wrap}{\mathtt{wrap}}
\newcommand{\clear}{\mathtt{clear}}
\newcommand{\src}{\mathtt{src}}
\newcommand{\thread}{\mathsf{thr}}
\newcommand{\op}{\mathsf{op}}
\newcommand{\trnsc}{\mathsf{txn}}
\newcommand{\crit}[1]{\mathsf{CS}_{#1}}
\newcommand{\addfresh}{\mathsf{addFresh}}


\newcommand{\set}[1]{\{#1\}}
\newcommand{\setpred}[2]{\{#1 \,|\, #2\}}
\newcommand{\tuple}[1]{\langle #1 \rangle}

\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * mathb
      <10.95> mathb10 <12> <14.4> <17.28> <20.74> <24.88> mathb12
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}
% \DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"88}
% \DeclareMathSymbol{\varsqsubsetneq} {3}{mathb}{"8A}
% \DeclareMathSymbol{\varsqsubsetneqq}{3}{mathb}{"92}
\DeclareMathSymbol{\sqsubsetneq}    {3}{mathb}{"8A}

\newcommand{\ord}[2]{\leq^{#1}_{\mathsf{#2}}}
\newcommand{\trord}[1]{\leq^{#1}_{\mathsf{tr}}}
% \newcommand{\stricttrord}[1]{<^{#1}_{\mathsf{tr}}}
% \newcommand{\tho}[1]{\leq^{#1}_{\mathsf{TO}}}
% \newcommand{\stricttho}[1]{<^{#1}_{\mathsf{TO}}}
% \newcommand{\nottho}[1]{\not\leq^{#1}_{\mathsf{TO}}}
% \newcommand{\stricttrord}[1]{<^{#1}_{\mathsf{tr}}}
\newcommand{\hb}[1]{\leq^{#1}_{\mathsf{HB}}}
\newcommand{\chb}[1]{\leq^{#1}_{\mathsf{CHB}}}
%\newcommand{\thb}[1]{<^{#1}_{\mathsf{THB}}}
\newcommand{\thb}[1]{\lessdot^{#1}_{\mathsf{Txn}}}
% \newcommand{\pth}[1]{\stackrel{*, #1}{\longrightarrow}}
\newcommand{\pth}[1]{\stackrel{*}{\longrightarrow_{#1}}}
\newcommand{\nedg}[1]{\lessdot^{#1}_{\mathsf{E}}}
\newcommand{\wcp}[1]{\leq^{#1}_{\mathsf{WCP}}}
\newcommand{\notwcp}[1]{\not\leq^{#1}_{\mathsf{WCP}}}
\newcommand{\strictwcp}[1]{\prec^{#1}_{\mathsf{WCP}}}
\newcommand{\ccp}[1]{\leq^{#1}_{\mathsf{DCP}}}
\newcommand{\notccp}[1]{\not\leq^{#1}_{\mathsf{DCP}}}
\newcommand{\strictccp}[1]{\prec^{#1}_{\mathsf{DCP}}}
\newcommand{\conc}[2]{\,||^{#1}_{\mathsf{#2}}\,}
\newcommand{\wcpconc}[1]{\,||^{#1}_{\mathsf{WCP}}\,}
\newcommand{\ccpconc}[1]{\,||^{#1}_{\mathsf{DCP}}\,}

\newcommand{\ccprank}[2]{\mathsf{rank}_\mathsf{DCP}^{#1}(#2)}
\newcommand{\wcprank}[2]{\mathsf{rank}_\mathsf{WCP}^{#1}(#2)}

\newcommand{\synctr}[1]{\mathsf{syncTrace}(#1)}
\newcommand{\unsynctr}[1]{\mathsf{unSyncTrace}(#1)}
\newcommand{\synctrev}[2]{\mathsf{syncTrace}^{#2}(#1)}
\newcommand{\freshvar}{\mathsf{fvar}}
\newcommand{\fsync}{\mathsf{first}\sync}
\newcommand{\lsync}{\mathsf{last}\sync}

\newcommand{\lw}[1]{\mathsf{lw}_{#1}}
\newcommand{\proj}[2]{#1|_{#2}}

\newcommand{\rtext}[1]{\textcolor{orange}{\sout{#1}}}
\newcommand{\atext}[1]{\textcolor{blue}{#1}}
\newcommand{\qtext}[1]{\textcolor{green}{#1}}

\newcommand{\ucomment}[1]{\textcolor{red}{#1}}
\newcommand\mycommfont[1]{\ttfamily{#1}}
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\newcommand{\cre}{\mathsf{CR}}

\renewcommand{\emptyset}{\varnothing}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}

% \theoremstyle{remark}
% \newtheorem{remark}{Remark}


\newcommand{\algo}{\text{AeroDrome}}
\newcommand{\tool}{\textsc{Rapid}}

\input{exec_macros}
\input{pseudocode_macros}

\newcommand{\trzero}{\rho_1}
\newcommand{\trone}{\rho_2}
\newcommand{\trtwo}{\rho_3}
\newcommand{\trthree}{\rho_4}
\newcommand{\trfour}{\rho_8}
\newcommand{\trfive}{\rho_9}
\newcommand{\trsix}{\rho_6}
\newcommand{\trseven}{\rho_7}
\newcommand{\treight}{\rho_5}
\newcommand{\trnine}{\rho_{10}}
\newcommand{\trten}{\rho_{11}}

% \newcommand{\nest}[2]{\mathtt{nest}(#1\!\rightarrow\! #2)}
\newcommand{\nest}[2]{\mathtt{nest}(#1,#2)}
% \newcommand{\figevnest}[3]{\figev{#1}{ \nest{#2}{#3} } }
\newcommand{\figevnest}[3]{ \figev{#1}{\acq(#2)}\figev{#1}{\acq(#3)}\figev{#1}{\rel(#3)}\figev{#1}{\rel(#2)} }

\newcommand{\nats}{\mathbb{N}}
\newcommand{\toolname}{\textsc{DeadTrack}~}
\newcommand{\lhist}{\mathsf{History}}

\newcommand{\djitp}{\textsc{Djit}+}

% \newcommand{\vc}[1]{\!\texttt{#1}\!}
\newcommand{\vc}[1]{\text{$\langle${\texttt{#1}}$\rangle$}}



==> pseudocode_macros.tex <==
%!TEX root = main.tex

\newcommand{\mx}{\sqcup}
\newcommand{\cle}{\sqsubseteq}
\newcommand\Ll{\mathbb{L}}
\newcommand{\Cc}{\mathbb{C}}
\newcommand{\Pp}{\mathbb{P}}
\newcommand{\Rr}{\mathbb{R}}
\newcommand{\Ww}{\mathbb{W}}
\newcommand\rth{\textsf{rThreads}}
\newcommand\wth{\textsf{LWT}}

\newcommand{\chL}{\mathbbm{ch}\mathbb{L}}
\newcommand{\chR}{\mathbbm{ch}\mathbb{R}}
\newcommand{\chW}{\mathbbm{ch}\mathbb{W}}

\newcommand{\lastw}{\mathsf{lastWThr}}
\newcommand{\lastrel}{\mathsf{lastRelThr}}
\renewcommand{\nil}{\mathtt{NIL}}

\newcommand{\upset}{\mathsf{UpdateSet}}
\newcommand{\stale}{\mathsf{Stale}}
\newcommand{\parenttr}{\mathsf{parentTr}}
\newcommand{\true}{\top\!\!\!\!\top}
\newcommand{\false}{\bot\!\!\!\!\bot}
